The Stability of Roll-Waves in Two-Phase Pipe Flow

Roll-wave trains constitutes a well-known two-phase flow regime in pipes. There exists a one-parameter family of steady roll-wave train solutions, provided the flow conditions are within the roll-wave range. This means that wave train solutions can be constructed from out of a wide range of wavelengths. That band of wavelengths which will be observed in nature is however fairly narrow. The wavelength distribution is believed to be related to wave train stability and the flow disturbances. Steady roll-wave train solutions are in this article subjected to a linear stability analysis. Comparisons are made with predictions from direct numerical Roe scheme simulations. Good agreement is observed; after an initial stage of wave coalescence, simulated wavelengths are distributed among the shorter of those wavelengths which are predicted linearly stable. Also the observed disturbance frequency and rate of decay agrees with the analysis predictions. Finally, the stability of pressure driven gas-liquid trains is compared to that of gravity driven free surface trains.

==> nomenclature.tex <==

% Latin
\nomenclature[Aa0]{$a,A$ }{Cross-sectional area \nomunit{m^2} }%
\nomenclature[Au0]{$u,U$ }{Fluid velocity \nomunit{m\,s^\textrm{-1}} }%
\nomenclature[Au1]{$\mc U$ }{Mixture velocity \nomunit{m\,s^\textrm{-1}} }%
\nomenclature[Af0]{$\bm f,\bm F$ }{Flux term  }%
\nomenclature[Af1]{$\tilde {\bm f}, \tilde{\bm F}$ }{Relative flux term }%
\nomenclature[As0]{$s,S$ }{Source  }%
\nomenclature[Ax0]{$x,X$ }{Spatial position }%
\nomenclature[At0]{$t$ }{Time  }%
\nomenclature[At0]{$\kk,\K$ }{Discharge rate (relative `mass flux') \nomunit{m^3\,s^\textrm{-1}} }%
\nomenclature[At0]{$c,C$ }{Shock speed/translation velocity \nomunit{m\,s^\textrm{-1}} }%
\nomenclature[At0]{$\j,\J$ }{Relative `momentum flux' \nomunit{kg\,m^\textrm{-1}\,s^\textrm{-2}} }%
\nomenclature[Ad0]{$d$ }{Diameter \nomunit{m} }%
\nomenclature[Ah0]{$h,H$ }{Height of interphase in pipe cross section \nomunit{m} }%
\nomenclature[Ah0]{$\H$ }{Hydraulic height $=A\l/\mr d_H A\l$ \nomunit{m} }%A\l'\of H
\nomenclature[Ar0]{$\mc R_0$ }{Profile reconstruction function }
\nomenclature[Am0]{$m\_x$ }{Interfacial friction multiplier}
\nomenclature[Ag0]{$g$ }{Gravitational acceleration \nomunit{m\,s^\textrm{-1}}}

%Greek
\nomenclature[B08]{$\theta$}{Pipe inclination \nomunit{-} }%
\nomenclature[B08]{$\theta$}{Pipe inclination \nomunit{-} }%
\nomenclature[B17]{$\rho$}{Density \nomunit{kg\, m^\textrm{-3} }}%
\nomenclature[B11]{$\lambda,\Lambda$}{Friction factor \nomunit{-} }%
\nomenclature[B11]{$\lambda^\pm,\Lambda^\pm$}{Eigenvalues }%
\nomenclature[B19]{$\tau, \mc T$ }{Skin friction \nomunit{kg\,m^\textrm{-1}\,s^\textrm{-2}} }
%\nomenclature[B031]{$\gamma\^m, \Gamma\^m$}{Mass source \nomunit{kg\,s^\textrm{-1}}}
%\nomenclature[B032]{$\gamma\^u, \Gamma\^u$}{Momentum source \nomunit{m\, kg\,s^\textrm{-2}}}
\nomenclature[B23]{$\bm \psi, \bm \Psi$}{Conservative state variables}
\nomenclature[B21]{$\phi$}{Symbolic variable}
\nomenclature[B19]{$\sigma, \Sigma$}{Peripheral area \nomunit{m^2}}

% Subscripts
\nomenclature[Ck]{$\kk$}{Generic phase: $\kappa\in\{\mathrm{g,\ell}\}$}%
\nomenclature[Cl]{$\ell$}{Liquid}%
\nomenclature[Cg]{$\mr g$}{Gas}%
\nomenclature[CL]{$\mr L$}{Left face of control volume}%
\nomenclature[CR]{$\mr R$}{Right face of control volume}%

% Superscripts
\nomenclature[Dn]{ $(n)$ }{Time iteration}%
\nomenclature[Ds]{ $\mr S$ }{`Superficial'; $\phi\k\^S = a\k/a \cdot \phi\k$}%
\nomenclature[D0p]{ $\pm$ }{Left or right side of a shock}%

% Encasements
\nomenclature[E01]{$\diffx \cdot$ }{$(\cdot)\_R-(\cdot)\_L$}% 
\nomenclature[E02]{$\difft \cdot$ }{$(\cdot)\n-(\cdot)\nm$}%
\nomenclature[E03]{$\diffk \cdot$ }{$(\cdot)\l-(\cdot)\g$}% 
\nomenclature[E04]{$\diff{ \cdot}_\pm$ }{$(\cdot)^+-(\cdot)^-$}% 
\nomenclature[E05]{$\ol{(\cdot)}$ }{Spatial average}% 
\nomenclature[E06]{$\an{(\cdot)}$ }{Temporal average}% 

%abbreviations

